An Understanding of the Shoulder of Giants: Jovian Planets around Late K Dwarf Stars and the Trend with Stellar Mass

Analyses of exoplanet statistics suggest a trend of giant planet occurrence with host star mass, a clue to how planets like Jupiter form. One missing piece of the puzzle is the occurrence around late K dwarf stars (masses of 0.5-0.75Msun and effective temperatures of 3900-4800K). We analyzed four years of Doppler radial velocities data of 110 late K dwarfs, one of which hosts two previously reported giant planets. We estimate that 4.0+/-2.3% of these stars have Saturn-mass or larger planets with orbital periods <245d, depending on the planet mass distribution and RV variability of stars without giant planets. We also estimate that 0.7+/-0.5% of similar stars observed by Kepler have giant planets. This Kepler rate is significantly (99% confidence) lower than that derived from our Doppler survey, but the difference vanishes if only the single Doppler system (HIP 57274) with completely resolved orbits is considered. The difference could also be explained by the exclusion of close binaries (without giant planets) from the Doppler but not Kepler surveys, the effect of long-period companions and stellar noise on the Doppler data, or an intrinsic difference between the two populations. Our estimates for late K dwarfs bridge those for solar-type stars and M dwarfs and support a positive trend with stellar mass. Small sample size precludes statements about finer structure, e.g. a "shoulder" in the distribution of giant planets with stellar mass. Future surveys such as the Next Generation Transit Survey and the Transiting Exoplanet Satellite Survey will ameliorate this deficiency.

==> table2_old.tex <==
\begin{deluxetable}{lrlrrrrrr}
\tabletypesize{\scriptsize}
\tablecaption{Stars Included in the Analysis\label{tab.stars}}
\tablewidth{0pt}

\tablehead{\colhead{Name} & \colhead{{\it V-J}} & \colhead{$T_{\rm eff}$ (K)} & \colhead{[Fe/H]} & \colhead{$S$} & \colhead{$M$ ($M_{\odot}$)} & \colhead{$N_{\rm obs}$} & \colhead{RMS (m s$^{-1}$)} & \colhead{$p^1$}}
\startdata
    HIP 1078 & 2.13 & 4426$^{b}$ & --- & 0.49 & 0.75 &   4 &   2.56       & 0.005 \\
    HIP 1532 & 2.52 & 3956$^{a}$ & -0.37 & 0.84 & 0.64 &  24 &   4.28       & 0.011 \\
    HIP 2247 & 2.06 & 4680$^{ }$ &  0.24 & 0.62 & 0.77 &  12 &   0.00       & 0.000 \\
    HIP 3418 & 2.16 & 4546$^{ }$ &  0.02 & 0.50 & 0.73 &   5 &   1.54       & 0.004 \\
    HIP 4353 & 2.20 & 4587$^{ }$ &  0.17 & 0.70 & 0.77 &   6 &  12.89       & 0.961 \\
    HIP 4454 & 1.99 & 4671$^{ }$ & -0.55 & 0.35 & 0.71 &   5 &   3.62       & 0.004 \\
    HIP 4845 & 2.58 & 4170$^{ }$ & -0.19 & 1.67 & 0.63 &  33 &   3.55       & 0.005 \\
    HIP 5247 & 2.51 & 4260$^{ }$ & -0.22 & 0.63 & 0.66 &  12 &   7.76       & 0.052 \\
    HIP 5663 & 2.34 & 4357$^{ }$ & -0.05 & 1.04 & 0.68 &  24 &   0.00       & 0.000 \\
    HIP 6344 & 2.32 & 4383$^{ }$ & -0.04 & 0.99 & 0.68 &   5 &   1.71       & 0.007 \\
    HIP 9788 & 2.15 & 4444$^{ }$ & -0.37 & 0.73 & 0.67 &  17 &   4.53       & 0.008 \\
   HIP 10337 & 2.54 & 4019$^{a}$ &  0.12 & 1.58 & 0.66 &  22 &   7.74       & 0.019 \\
   HIP 10416 & 1.88 & 4743$^{ }$ &  0.14 & 0.71 & 0.76 &  11 &  10.43       & 0.721 \\
   HIP 11000 & 1.92 & 4703$^{ }$ &  0.20 & 0.76 & 0.73 &  13 &  10.54       & 0.195 \\
   HIP 12493 & 2.25 & 4350$^{ }$ & -0.29 & 0.66 & 0.68 &   6 &   4.50       & 0.032 \\
   HIP 13375 & 2.50 & 4110$^{b}$ &  0.00 & 0.59 & 0.56 &   9 &   3.68       & 0.010 \\
   HIP 14729 & 2.15 & 4579$^{ }$ &  0.17 & 1.00 & 0.70 &  10 &   5.76$^{c}$ & 0.007 \\
   HIP 15095 & 2.28 & 4265$^{ }$ & -0.21 & 1.28 & 0.68 &  10 &   6.82       & 0.071 \\
   HIP 15563 & 2.06 & 4718$^{ }$ &  0.16 & 1.04 & 0.72 &  12 &  10.74       & 0.332 \\
   HIP 15673 & 1.93 & 4654$^{ }$ & -0.46 & 0.50 & 0.69 &   6 &   3.12       & 0.007 \\
1234-00069-1 & 1.90 & 4657$^{b}$ & --- & 0.42 & 0.75 &   4 &   1.30       & 0.023 \\
   HIP 17346 & 2.06 & 4613$^{ }$ &  0.07 & 0.59 & 0.74 &   6 &   4.19       & 0.012 \\
   HIP 17496 & 2.15 & 4489$^{ }$ & -0.04 & 0.62 & 0.72 &   5 &   2.53       & 0.008 \\
   HIP 19165 & 2.24 & 4412$^{ }$ & -0.22 & 0.64 & 0.65 &  31 &   5.16       & 0.010 \\
   HIP 19981 & 2.25 & 4605$^{ }$ &  0.27 & 0.70 & 0.77 &   5 &   4.60       & 0.017 \\
   HIP 20359 & 2.14 & 4547$^{ }$ & -0.04 & 0.58 & 0.75 &   5 &   4.47       & 0.011 \\
   HIP 25220 & 2.04 & 4613$^{ }$ &  0.05 & 0.89 & 0.71 &  10 &   7.92       & 0.049 \\
   HIP 26196 & 2.34 & 4245$^{b}$ & --- & 0.76 & 0.74 &   8 &   4.26$^{d}$ & 0.012 \\
4356-01014-1 & 1.88 & 4737$^{ }$ & -0.17 & 0.46 & 0.77 &   8 &   2.69       & 0.003 \\
   HIP 29548 & 2.32 & 4528$^{ }$ & -0.10 & 0.59 & 0.69 &  20 &   3.79       & 0.006 \\
   HIP 30112 & 2.36 & 4226$^{b}$ & --- & 1.46 & 0.72 &  25 &   7.45       & 0.040 \\
   HIP 30979 & 2.02 & 4627$^{ }$ &  0.23 & 0.60 & 0.77 &  12 &   5.41       & 0.005 \\
3388-01009-1 & 2.36 & 4220$^{b}$ & --- & 1.38 & 0.68 &  10 &  64.66       & 0.500 \\
   HIP 32769 & 2.24 & 4420$^{ }$ & -0.05 & 0.68 & 0.71 &  16 &   4.86       & 0.005 \\
   HIP 32919 & 2.33 & 4382$^{ }$ & -0.01 & 0.86 & 0.70 &  18 &   5.29       & 0.006 \\
1352-01588-1 & 2.31 & 4270$^{b}$ & --- & 0.00 & 0.69 &   7 &  18.27       & 0.918 \\
0748-01711-1 & 2.50 & 4108$^{b}$ & --- & 0.16 & 0.66 &  25 &  42.28$^{c}$ & 0.500 \\
   HIP 36551 & 2.09 & 4501$^{ }$ & -0.30 & 0.57 & 0.70 &  11 &   3.86       & 0.007 \\
   HIP 37798 & 2.54 & 4082$^{b}$ & --- & 1.42 & 0.70 &   9 &   3.12       & 0.005 \\
   HIP 38969 & 2.13 & 4761$^{ }$ &  0.26 & 0.40 & 0.81 &  10 &  10.96$^{c}$ & 0.817 \\
   HIP 40375 & 2.18 & 4463$^{ }$ &  0.03 & 0.96 & 0.71 &  33 &   6.67       & 0.009 \\
   HIP 40671 & 2.05 & 4612$^{ }$ &  0.06 & 0.46 & 0.74 &   6 &   1.95       & 0.008 \\
   HIP 40910 & 2.41 & 4256$^{ }$ & -0.06 & 1.41 & 0.68 &  21 &   9.47       & 0.665 \\
   HIP 41130 & 2.26 & 4410$^{ }$ & -0.10 & 1.10 & 0.72 &  18 &   8.46       & 0.603 \\
   HIP 41443 & 2.08 & 4613$^{ }$ &  0.01 & 0.83 & 0.74 &   9 &   6.10       & 0.014 \\
   HIP 42567 & 1.94 & 4648$^{ }$ &  0.09 & 0.71 & 0.76 &   6 &   6.00       & 0.037 \\
   HIP 43534 & 2.56 & 4100$^{a}$ & -0.13 & 1.49 & 0.64 &  14 &   6.88       & 0.006 \\
   HIP 43667 & 2.12 & 4554$^{ }$ &  0.01 & 0.51 & 0.72 &   9 &   5.24       & 0.020 \\
   HIP 44072 & 2.16 & 4347$^{ }$ & -0.42 & 0.52 & 0.71 &   5 &   3.96       & 0.020 \\
   HIP 45042 & 2.35 & 4476$^{ }$ &  0.17 & 1.27 & 0.73 &   5 &   9.94       & 0.095 \\
1955-00658-1 & 2.52 & 4493$^{ }$ &  0.21 & 1.48 & 0.66 &   4 &   6.05       & 0.055 \\
   HIP 45839 & 2.12 & 4590$^{ }$ &  0.05 & 0.55 & 0.72 &   5 &  12.40       & 0.865 \\
   HIP 46343 & 2.20 & 4529$^{ }$ &  0.03 & 1.03 & 0.70 &  10 &   4.35       & 0.008 \\
   HIP 46417 & 2.28 & 4475$^{ }$ & -0.06 & 0.69 & 0.71 &   9 &   7.19       & 0.018 \\
   HIP 47201 & 2.37 & 4376$^{ }$ &  0.03 & 0.98 & 0.69 &   7 &   4.91       & 0.045 \\
   HIP 48139 & 2.09 & 4548$^{a}$ &  0.22 & 0.45 & 0.77 &   6 &   2.34       & 0.004 \\
   HIP 48411 & 2.14 & 4505$^{ }$ &  0.20 & 0.78 & 0.73 &   4 &   8.32       & 0.057 \\
   HIP 48740 & 2.22 & 4577$^{ }$ &  0.02 & 1.10 & 0.72 &   8 &   7.38       & 0.015 \\
   HIP 50960 & 2.40 & 4187$^{a}$ & -0.06 & 1.51 & 0.65 &   8 &   8.22       & 0.023 \\
   HIP 51443 & 2.16 & 4505$^{ }$ & -0.05 & 1.09 & 0.71 &  19 &   8.56       & 0.447 \\
   HIP 53327 & 2.29 & 4390$^{ }$ & -0.79 & 0.37 & 0.66 &   4 &   5.13       & 0.018 \\
   HIP 54459 & 2.26 & 4469$^{ }$ & -0.52 & 0.37 & 0.68 &  13 &   8.32       & 0.028 \\
   HIP 54651 & 2.11 & 4395$^{ }$ & -0.89 & 0.33 & 0.66 &   6 &   1.63       & 0.002 \\
   HIP 54810 & 2.09 & 4530$^{ }$ &  0.03 & 1.04 & 0.70 &   5 &   6.18       & 0.061 \\
   HIP 55507 & 2.42 & 4404$^{ }$ & -0.05 & 0.90 & 0.69 &  22 &   6.37$^{c}$ & 0.013 \\
   HIP 56630 & 2.67 & 3983$^{a}$ & -0.01 & 1.37 & 0.68 &   9 &   7.29       & 0.045 \\
   HIP 57274 & 2.00 & 4641$^{ }$ &  0.08 & 0.39 & 0.76 & 120 &   0.00       & 1.000 \\
   HIP 57493 & 2.38 & 4372$^{ }$ &  0.06 & 1.16 & 0.71 &  15 &   5.48       & 0.009 \\
   HIP 59496 & 2.41 & 4344$^{ }$ & -0.01 & 1.42 & 0.69 &   7 &   9.67       & 0.203 \\
   HIP 60633 & 2.08 & 4724$^{ }$ &  0.25 & 0.33 & 0.76 &  26 &  12.92       & 1.000 \\
   HIP 62406 & 2.38 & 4527$^{ }$ &  0.31 & 1.10 & 0.68 &  39 &   8.07       & 0.118 \\
   HIP 62847 & 1.97 & 4726$^{ }$ &  0.05 & 0.66 & 0.81 &  34 &   6.03       & 0.012 \\
   HIP 63894 & 2.20 & 4361$^{b}$ & --- & 0.81 & 0.69 &   8 &   6.47       & 0.029 \\
   HIP 64048 & 2.17 & 4615$^{ }$ &  0.08 & 0.71 & 0.71 &  14 &   8.63       & 0.029 \\
   HIP 64262 & 2.03 & 4639$^{ }$ & -0.25 & 0.59 & 0.70 &   9 &   8.13       & 0.047 \\
   HIP 66074 & 2.32 & 4460$^{ }$ &  0.23 & 1.17 & 0.73 &   9 &  11.06       & 0.818 \\
   HIP 66222 & 2.71 & 4157$^{ }$ & -0.11 & 1.34 & 0.68 &  13 &   6.54       & 0.017 \\
   HIP 66283 & 1.84 & 4880$^{ }$ &  0.18 & 0.00 & 0.84 &   7 &  10.71       & 0.256 \\
   HIP 66840 & 2.47 & 4138$^{b}$ & --- & 0.00 & 0.69 &   5 &   1.96       & 0.008 \\
   HIP 67842 & 2.76 & 3919$^{b}$ & --- & 1.23 & 0.64 &   6 &   5.18       & 0.016 \\
   HIP 73427 & 2.40 & 4337$^{ }$ & -0.02 & 1.26 & 0.73 &  11 &  13.32       & 0.949 \\
   HIP 75672 & 2.45 & 4149$^{b}$ & --- & 0.00 & 0.69 &   4 &   2.67       & 0.021 \\
   HIP 77908 & 2.27 & 4612$^{ }$ &  0.28 & 0.98 & 0.74 &   5 &   2.50       & 0.008 \\
   HIP 78184 & 2.47 & 4130$^{b}$ & --- & 0.00 & 0.68 &   4 &   7.08       & 0.004 \\
   HIP 78999 & 2.05 & 4504$^{ }$ &  0.24 & 0.00 & 0.73 &   4 &   6.30       & 0.029 \\
   HIP 79698 & 2.31 & 4513$^{ }$ &  0.26 & 0.91 & 0.74 &   7 &   3.51       & 0.004 \\
   HIP 87464 & 2.17 & 4417$^{ }$ & -0.27 & 0.44 & 0.69 &   8 &   8.76       & 0.351 \\
   HIP 89087 & 2.40 & 4329$^{ }$ & -0.01 & 1.38 & 0.68 &   4 &   3.48       & 0.001 \\
   HIP 93871 & 2.06 & 4453$^{a}$ & -0.47 & 0.28 & 0.71 &   4 &   3.38       & 0.001 \\
   HIP 97051 & 2.34 & 4320$^{ }$ & -0.19 & 1.10 & 0.62 &  19 &   9.10       & 0.183 \\
   HIP 99205 & 2.15 & 4397$^{ }$ & -0.18 & 0.85 & 0.64 &   6 &   6.32       & 0.021 \\
   HIP 99332 & 2.15 & 4400$^{a}$ &  0.30 & 0.73 & 0.76 &   8 &   5.82       & 0.033 \\
  HIP 101262 & 2.06 & 4774$^{ }$ &  0.19 & 1.00 & 0.73 &   4 &   9.06       & 0.146 \\
  HIP 102332 & 2.39 & 4202$^{b}$ & --- & 0.75 & 0.66 &   4 &   5.56       & 0.017 \\
  HIP 103650 & 2.10 & 4603$^{ }$ & -0.04 & 0.75 & 0.71 &   9 &   5.22       & 0.020 \\
  HIP 104092 & 2.23 & 4455$^{ }$ &  0.07 & 0.54 & 0.72 &   5 &   6.66       & 0.057 \\
  HIP 105341 & 2.55 & 4299$^{ }$ & -0.05 & 1.38 & 0.68 &   5 &   8.68       & 0.087 \\
  HIP 109980 & 2.14 & 4580$^{ }$ &  0.00 & 0.95 & 0.71 &  56 &   6.73       & 0.024 \\
  HIP 110774 & 2.14 & 4471$^{ }$ & -0.12 & 0.87 & 0.67 &   4 &   1.91       & 0.000 \\
3995-01436-1 & 2.16 & 4634$^{ }$ &  0.08 & 0.89 & 0.71 &   9 &   7.20       & 0.051 \\
  HIP 112496 & 2.00 & 4778$^{ }$ &  0.04 & 0.65 & 0.75 &   5 &   7.92       & 0.059 \\
  HIP 112918 & 2.26 & 4434$^{ }$ &  0.02 & 1.20 & 0.67 &   4 &   2.80       & 0.018 \\
  HIP 114156 & 2.45 & 4322$^{ }$ & -0.02 & 1.43 & 0.66 &   4 &   3.41       & 0.025 \\
  HIP 115004 & 2.22 & 4684$^{ }$ & -0.11 & 0.83 & 0.82 &  21 &  40.79$^{c}$ & 0.500 \\
  HIP 117197 & 2.56 & 4153$^{ }$ & -0.38 & 1.05 & 0.61 &  19 &   3.15       & 0.002 \\
  HIP 117492 & 2.10 & 4679$^{ }$ &  0.08 & 0.98 & 0.73 &   5 &   5.09       & 0.029 \\
  HIP 117559 & 2.25 & 4581$^{ }$ &  0.07 & 1.28 & 0.71 &  41 &   9.82       & 0.447 \\
  HIP 117946 & 1.95 & 4863$^{ }$ &  0.03 & 0.85 & 0.77 &  14 &   9.00       & 0.143 \\
  HIP 118261 & 1.90 & 4662$^{ }$ & -0.04 & 0.65 & 0.74 &  34 &   7.28       & 0.025 \\
  HIP 118310 & 2.24 & 4326$^{b}$ & --- & 0.71 & 0.80 &   4 &   0.00       & 0.000 \\
\enddata
\tablenotetext{a}{based on medium-resolution spectroscopy}
\tablenotetext{b}{based on $V-J$ color}
\tablenotetext{c}{a linear trend removed}
\tablenotetext{d}{a parabolic trend removed}
\end{deluxetable}

